SPIRE: Synergistic Planning, Imitation, and Reinforcement Learning for Long-Horizon Manipulation

Robot learning has proven to be a general and effective technique for programming manipulators. Imitation learning is able to teach robots solely from human demonstrations but is bottlenecked by the capabilities of the demonstrations. Reinforcement learning uses exploration to discover better behaviors; however, the space of possible improvements can be too large to start from scratch. And for both techniques, the learning difficulty increases proportional to the length of the manipulation task. Accounting for this, we propose SPIRE, a system that first uses Task and Motion Planning (TAMP) to decompose tasks into smaller learning subproblems and second combines imitation and reinforcement learning to maximize their strengths. We develop novel strategies to train learning agents when deployed in the context of a planning system. We evaluate SPIRE on a suite of long-horizon and contact-rich robot manipulation problems. We find that SPIRE outperforms prior approaches that integrate imitation learning, reinforcement learning, and planning by 35% to 50% in average task performance, is 6 times more data efficient in the number of human demonstrations needed to train proficient agents, and learns to complete tasks nearly twice as efficiently. View https://sites.google.com/view/spire-corl-2024 for more details.

==> todo.tex <==
------list of todos------------
1. writing

(1page) intro - ajay
    (see the outline in text)
    highlight the complexity in systemic combination with non-trivial design choices. 

(0.75) related work - animesh
    how we are diff from BC+Rl methods
        why don't we compare with GAIL or others. (rebuttal or supplement)
        why didn't you run fish -- BC warm start and then fine tune. 
            for just the stages we decompose - then bc + RL should work
            without planning RL would be 0\%,

(2.5) methods
prelims: 
    MDP/RL

our methods
    tamp - Caelan
        parameterized operators
        preconditions when rl starts for traje segmentation
    sequential short episodes. 
        choice of where to start/end    
        technical novelty of using tamp 
            need to differentiate from BC-> RL vanilla
    details of loss
        constraint on the deviation of loss from BC
    if we leverage parallel envs, how
    system components to enable rl in sequential tasks 
    
experiments
    setup
        teleop
        list of tasks and description in appendix
    baselines
        list and description in appendix
    metrics
        list and explanation

    analysis
        1 sentence bold takeaways

conclusions
    

----------------------
List of floats
link: https://nvidia-my.sharepoint.com/:p:/r/personal/zihanz_nvidia_com/Documents/rl-hitl-tamp.pptx?d=wdc66c15fd1c7483a8421866a4cc18d14&csf=1&web=1&e=NwSqtQ

Teaser - (page 2)    
    juxtapose with RL and BC
    method to showcase that this mixes

Algo figure - overview of the method (page 4)
    full pipeline
    hand off from tamp to rl
    train bc with tamp gating
    then finetune with rl

1-2 figures showing multi-worker TAMP

Qualitative results (page 5)
    what would this look like -- 
        overlay the keyframes
    bc is failing -- maybe OOD eval. 
    rl doing some dangerous action -- 

-----
1. table for main result - 
    or bar plots. 
        succ. rate, median episode length (for succ episodes only)

demo efficiency
    bar plot with x-axis as data (10-50-200)
    minimum number of demos to reach 70\% success rate in (Coffee, ThreePiece, Square)

breakdown of coffee prep (most complicated task)
    sequence of learned policies, deployed with tamp

ablation 
    divergence loss
    action vs fine tuning


---

populate appendix. 
    details of experimental setup
        details envs. 
        details of baselines
        teleop data collection?
        base algorithm (drqv2)
        network structure
    extensive evaluations
        * variance analysis & discussion - why we choose best
        * other demo + RL (gail, fish)
        * ablate TAMP
        object-state experiments
        error cases
        BC loss vs KL pen

other supplements
    rollout videos
    reset distribution
    3min overview video?
        how efficient ft vs bc
        per-section bc vs ft
        parallelization overview figure 

